From Adversarial Arms Race to Model-centric Evaluation: Motivating a Unified Automatic Robustness Evaluation Framework

Textual adversarial attacks can discover models' weaknesses by adding semantic-preserved but misleading perturbations to the inputs. The long-lasting adversarial attack-and-defense arms race in Natural Language Processing (NLP) is algorithm-centric, providing valuable techniques for automatic robustness evaluation. However, the existing practice of robustness evaluation may exhibit issues of incomprehensive evaluation, impractical evaluation protocol, and invalid adversarial samples. In this paper, we aim to set up a unified automatic robustness evaluation framework, shifting towards model-centric evaluation to further exploit the advantages of adversarial attacks. To address the above challenges, we first determine robustness evaluation dimensions based on model capabilities and specify the reasonable algorithm to generate adversarial samples for each dimension. Then we establish the evaluation protocol, including evaluation settings and metrics, under realistic demands. Finally, we use the perturbation degree of adversarial samples to control the sample validity. We implement a toolkit RobTest that realizes our automatic robustness evaluation framework. In our experiments, we conduct a robustness evaluation of RoBERTa models to demonstrate the effectiveness of our evaluation framework, and further show the rationality of each component in the framework. The code will be made public at \url{https://github.com/thunlp/RobTest}.

==> deficiency.tex <==

% \paragraph{Incomprehensive Evaluation and Inaccurate Claim.}



% \paragraph{Lacking Instruction for Robustness Evaluation. \yang{Need discussion}}
% We witness the rapid progress in adversarial NLP. 
% Many platforms and toolkits have been developed~\cite{morris-etal-2020-textattack, goel2021robustness, zeng-etal-2021-openattack, wang-etal-2021-textflint}, implementing many existing attack and defense algorithms. 
% These tools help researchers to quickly reproduce experimental results, thus speeding up the attack-and-defense competition. 
% However, when we seek more practical significance, we would want some instructions for how to evaluate models' robustness, besides a bunch of tools on display.
% We note one exception in Robustness gym~\cite{goel2021robustness}, which do provide guidance for evaluation. 
% However, the instructions are high-level, making them difficult to be comprehended for practitioners outside this field.

% To tackle this, we define general task-agnostic robustness dimensions in our paradigm. 
% We give our motivation and explanation for why we should measure these dimensions for users, and potential consequences of obtaining lower scores. 
% Thus, our paradigm can help users to gain a better understanding of their models.





% \paragraph{Pursuing Attacking Performance while Ignoring Sample Validity.}


% \paragraph{Unnecessary Restriction.}


% \paragraph{Inappropriate Adversarial Sample Selection Strategy.}
% \label{sec:deficiency}



==> tabs/compare_dimensions.tex <==
\begin{table}[htp]
\centering
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{lccc}
\toprule
Robustness Evaluation Framework  & Comprehensivenss & Reasonability & Reliability  \\ \midrule
Single Attack Method~\citep{zang-etal-2020-word} & \XSolidBrush               & $\textbf{P}$  & $\textbf{P}$ \\
Adversarial GLUE~\citep{wang2021adversarial}     & \XSolidBrush               &  \CheckmarkBold           &  \CheckmarkBold          \\
OpenAttack~\citep{zeng-etal-2021-openattack}           & $\textbf{P}$     & \XSolidBrush            & \XSolidBrush           \\
TextAttack~\citep{morris-etal-2020-textattack}           & $\textbf{P}$     & \XSolidBrush            & \XSolidBrush           \\
TextFlint~\citep{wang-etal-2021-textflint}            &  \CheckmarkBold              & $\textbf{P}$  & \XSolidBrush           \\
Robustness Gym~\citep{goel2021robustness}       & $\textbf{P}$     & $\textbf{P}$  & \XSolidBrush           \\
Challenging Dataset~\citep{nie2019adversarial}  & \XSolidBrush               & \CheckmarkBold   &  \CheckmarkBold          \\
Ours                 &  \CheckmarkBold              &  \CheckmarkBold           &  \CheckmarkBold          \\ \bottomrule
\end{tabular}
}
\caption{Comparison with previous robustness evaluation frameworks. $\textbf{P}$ indicates that the specific dimension can be partially met. \textit{Reasonability} measures whether the framework establishes a reasonable evaluation protocol that satisfies the practical needs. 
\textit{Reliability} measures whether the evaluated samples are valid.}
\label{tab: compar} 
\end{table}

==> tabs/human_eval_2.tex <==
\begin{table}[t]
\centering
\resizebox{0.47\textwidth}{!}{
\begin{tabular}{lllll}
\toprule
Method | Level & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{2} & \multicolumn{1}{c}{3} & \multicolumn{1}{c}{4} \\ \midrule
Grammar                     & 49.82                 & 67.81                 & 80.18                 & 71.45                 \\
USE                         & 78.18                 & 61.09                 & 71.27                 & 58.73                 \\
Perplexity                  & 66.00                 & 71.27                 & 69.63                 & 62.36                 \\
Degree                      & 80.55                 & 69.45                 & 62.55                 & 56.73                 \\ \bottomrule
\end{tabular}
}
\caption{\label{tab:human_eval_2} TMP
 }
\end{table}



==> tabs/perceptible_perturbation_cases.tex <==
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{ll}
\toprule
Original                                            & I \color[HTML]{000000} love the way that it took chances and really asks you to take these great leaps of faith and pays off.                 \\ \midrule
\multicolumn{1}{c}{Malicious Robustness Evaluation (Distraction)} & I \color[HTML]{000000} love the way that it took chances and really asks you to take these great leaps of faith and pays off.  \color[HTML]{FE0000} Down Down Down \\ \midrule
General Robustness Evaluation (Typo)                      & I \color[HTML]{000000} love the way that it took \color[HTML]{FE0000} chancs  \color[HTML]{000000} and really asks you to \color[HTML]{FE0000} takke \color[HTML]{000000} these great leaps of faith and pays off.           \\ \bottomrule     

\end{tabular}
}
\caption{\label{tab:perceptible_perturb_cases} 
Adversarial samples with perceptible perturbations.  }


\end{table*}


